On the (In)security of Peer-to-Peer Decentralized Machine Learning

In this work, we carry out the first, in-depth, privacy analysis of Decentralized Learning -- a collaborative machine learning framework aimed at addressing the main limitations of federated learning. We introduce a suite of novel attacks for both passive and active decentralized adversaries. We demonstrate that, contrary to what is claimed by decentralized learning proposers, decentralized learning does not offer any security advantage over federated learning. Rather, it increases the attack surface enabling any user in the system to perform privacy attacks such as gradient inversion, and even gain full control over honest users' local model. We also show that, given the state of the art in protections, privacy-preserving configurations of decentralized learning require fully connected networks, losing any practical advantage over the federated setup and therefore completely defeating the objective of the decentralized approach.

==> cl.tex <==
\subsection{Collaborative Machine Learning}
 Collaborative machine learning enables a set of $n$ distributed \textit{users} $V$ to train a shared model $f$ defined by a set of parameters $\Theta$. Each client $v \in V$ that participates in the training protocol with a set of training instances $X_v$. This training dataset must be kept private, i.e., it must not be directly shared and parties involved in the training should not learn anything about each other's training set besides what can be inferred from the final model. %In this paper, we limit our privacy definition to the privacy of this training set, and not other attributes that could be learned about users (e.g., location~\cite{locationprivacy} or device type).

The model $f$ is generally trained relying on a distributed version of Stochastic Gradient Descent (SGD), where information about users' training sets is iteratively propagated via \textit{model updates}. These updates are intermediate outputs of the local optimization process \ie gradients or parameters~\cite{fedavg, can_dec} obtained after one or more local SGD steps. Users receive updates from other users via direct connections in a peer-to-peer fashion (DL), or indirectly through other parties such as parameters server (FL).

\subsubsection{Federated Learning}
In federated learning~\cite{fedavg} users performs the distribute training process with the support  of a central \textit{parameter server} that iteratively aggregates and synchronizes model updates among users (Figure~\ref{fig:fl}). %The server manages users' training process and maintains a master copy of the global model's parameters within the training process.
%In the initial setup phase, users and server choose a training task and define a machine learning model.
%This model is initialized and hosted by the parameter server.
At each training step, users download the global model from the server and locally apply one or more local training steps. Users then send the generated model updates (\eg accumulated gradients or parameters) to the server that aggregates and applies them to the current global parameters, completing a training round.

%as the server has linear communication cost in the number of users.
As main consequence, in FL, there is no direct communication among users. Users, by design, do not have access to each other's model updates during the training; they can only access the final\mr{would rm final, can access per epoch} aggregated model update produced by the parameter server from which individual users' contributions cannot be distinguished\mr{is this true? thinking about broader privacy then MIA}. %While this still permit

\subsubsection{Decentralized Learning}
In DL, there is no central parameter server and users directly communicate with each other via  peer-to-peer channels. Those channels are generally modeled by an \textit{undirected} graph~$G$, where users are nodes and peer-to-peer communication channels are edges (Figure~\ref{fig:dl}). Hereafter, we refer to this graph as \textit{communication topology} or simply \textit{topology}.
\par

At each training step, users aggregate the model updates received from their \textit{neighbors}, locally apply one or more optimization steps using their local training dataset, and broadcast their adjusted model parameters (Figure~\ref{fig:dl}).
During these steps, \textbf{users have a local view of the current parameters different from other users} \mr{each user has local paramaters different from the other users}. This is in contrast with the classic federated learning model, where there is a single global set of parameters shared among all the users.
Eventually, after a suitable number of communication rounds, users find \textit{consensus} on a global set of parameters; that is, all the local models become equal.
\par

\new{As advocated by decentralized learning proposers, a core advantage offered by decentralized learning is that,  in contrast to federated learning \mr{where connections are fixed and centered around the server}, users can now choose with whom communicate during the training. For instance, this allows them to directly collaborate only with users with affine training sets and maximize utility on a target data distribution. \mr{-> too precise, would specify smh like "based either on similarity, trust, or computational management choices.""} In current works, no particular attention is paid in limiting \mr{not only limiting but more like managing, as long as the graph is connected} users' connectivity and/or enforcing pre-defined topologies. Thus, in the current state, decentralized users are enabled to arbitrarily pick the neighbor nodes \mr{-> create links arbritraly}.}
%\par


%\todo{ There exists a massive body of active studies on decentralized learning~\cite{bellet2018personalized, Blanchard17, DamaskinosMGPT18, el2020collaborative, he2022byzantine,Koloskova2020Decentralized, lalitha2019peer, lalitha2018fully, pappas2021ipls, pei2021decentralized, braint, Shokri15, vogels2021relaysum, can_dec, XiaoB04, Yin18, ying2021bluefog, yuan2021defed, ZhangXCF19}. These works improve different aspects of decentralized learning, among others scalability, asynchronicity and data heterogeneity.}


%Contrary to decentralized learning, in federate learning \textbf{users share the same global state throughout the whole training process}.
%Users receiving the update cannot distinguish neither the individual contributions nor their origin (\ie which user generated what).
%Once the server's network is updated, the clients download the new state of the model and repeat the protocol till a stop condition is reached.
%This process repeats till a stop condition is met.


==> hbc_defenses.tex <==
Next, we discuss defensive techniques that could be used to prevent the passive attacks introduced in this section.

\parabf{Topology Changes.}
%A first, already discussed, defense to reduce the leakage from model updates is to increase the density of the topology to global generalization (Section~\ref{sec:recmup}),
%reaching global generalization at every step if the communication topology is complete. However, density not only increases the communication cost, but makes users susceptible to gradient inversion attacks. Thus, this simple solution is not desirable.
Reducing the leakage {of model updates} originated from local generalization requires increasing the density of the communication topology underlying the decentralized learning network (Section~\ref{sec:recmup}). Ideally, the topology would be complete, minimizing local learning effects and thus leakage. Yet, such a decision is in conflict with the conclusions of Section~\ref{sec:passive_user_vs_server}, which show that increasing connectivity enhances the adversary's capability to collect knowledge of the system which results in even more significant inferences about other honest users' training sets. Indeed, with a complete topology, every user would reach the same adversarial capabilities of a passive parameter server in federated learning. We discuss in Section~\ref{sec:opm} future steps to alleviate problems associated to how the communication topology is built.


\parabf{Secure Aggregation.}
A way for decentralized learning to evade the local generalization vs. system-knowledge minimization trade-off is to rely on secure aggregation protocols (SA)~\cite{secagg}. In these protocols, every node implements the aggregation in line $8$ of Algorithm~\ref{alg:dl} in a privacy-preserving way, i.e., without revealing the values of their updates in the clear. Intuitively, preventing the attacker from accessing individual model updates would eliminating attacks relying on {system knowledge} such as gradient recovery and functional marginalization; although gradient recovery would unavoidably succeed when $\nn(\victm)\myeq\{\attck\}$ (always) or $\nn(\attck)\myeq\{\victm\}$ (when $C$ approaches zero).

Thus, when SA is applied, decentralized learning can grant users the same level of privacy against passive adversaries as federated learning by relying on a complete topology to achieve global generalization. While this may seem a suitable solution, every user in this setup has the same communication complexity as a parameter server in federated learning in addition to the overhead imposed by the cryptographic operations needed for secure aggregation. At such point, deploying secure aggregation-based decentralized learning results on a massive overhead with respect to federated learning at no gain in privacy. This essentially contradicts the premises behind the development of decentralized learning protocols, casting doubt on their utility.


\parabf{Other mitigations.}
%An alternative solution to reduce the effect of local generalization could be the decentralized learning protocol proposed by Vogels \etal~to handle data heterogeneity~\cite{vogels2021relaysum}. In this protocol, users propagate the \textit{exact} model updates of other users. This approach effectively creates phantom/virtual edges between users routing model updates through non-neighbors nodes, and thus it does not solve the underlying problem. In fact, this setup only increases the power of active adversaries that now can not only influence others with their own updates, but also by manipulating other users' updates (see Section~\ref{sec:influence_factor}).%\footnote{Plus, adversaries are also granted with the knowledge of the global communication topology needed to compute the required spanning tree, unless a centralized entity is considered.\ct{i don't understand what this footnote brings. But either it is important enough to be in the main text, or it should go}}
%\ct{this second part I cannot follow. We need more concreteness. It is clear in your head but not here.} However, this would not solve completely the privacy risk intrinsic in the model updates and the underlying local generalization phenomenon. Indeed, as for generalization, the privacy offered by SA scales with the number of users participating to the protocol. This means that  sparsely connected attackers would be always able to infer more information from the aggregated model updates than what is possible in federated learning. %Despite all this, even if SA can drastically reduce the advantage of a decentralized attacker, it is not clear if this can be meaningfully implemented in the decentralized setting (see Section~\ref{sec:sa}).
%A trivial solution to counter gradient recovery would be to rely on \textit{model inconsistency}~\cite{evading_sec}, where users distribute slightly different versions of the same model to their neighbors (\eg by adding noise independently sampled for each neighbor user). This approach would  prevent perfect gradient recovery, inducing an error proportional to the discrepancy among the distributed models. However, this would result in a non-negligible impact on the convergence rate of the consensus-based system. More research is needed to understand whether there is an operation point in which attacks can be thwarted to a large extent while still obtaining a performance that improves the trade-offs in federated learning.
\new{We acknowledge that approaches such as gradient compression~\cite{\jaggi} (and similar~\cite{pmlr-v162-dai22b}) may be functional in reducing the amount of information in the shared model updates, and thus (purely informally~\cite{gobfs}) would decrease the privacy risk associated to the shared models~\cite{huang2021evaluating}. A consistently more principled defense, instead, would be using differential private SGD. We discuss this option in Section~\ref{sec:dp}. However, all these \textit{gradient-perturbation}-based techniques can be also applied in federated learning and thus do not result in any advantage for the decentralized setting; that is, they cannot close the security gap between DL and FL.}% \new{In other words, these techniques would not close the security gap standing in between decentralized and federated learning.}
%\ct{I also do not understand this. Privacy is increased in FL? what is the point?} As we show in Section~\ref{sec:dp}, in federated learning, the privacy properties induced by these techniques would be just amplified by the non-sparse aggregation performed by the server.


==> mlc_defenses.tex <==
Next, we discuss  defensive techniques that could be used to prevent the active attacks introduced in this section.

\parabf{Topology Changes.}
Adversarial influence is enabled by the same decentralized learning characteristics as local generalization. Therefore, the same defenses apply: the best way to reduce the influence power of an active attacker is to increase the number of neighbors of each node, diluting the influence of malicious neighbors. But increasing the topology density puts malicious neighbors in an advantage position to  collect information about the global state of the system, enabling them to run \textit{state-override} attacks (Section~\ref{sec:override}). %We discuss in Section~\ref{sec:sa} possible ways to mitigate problems associated to the communication topology.
%In Section~\ref{sec:override}, we demonstrate that such adversarial knowledge translates in a even more critical security issue in the malicious setting.
%\par

\parabf{Secure Aggregation.}
Secure aggregation can prevent system-knowledge-based attacks such as the echo and state override attacks. However, SA does not solve the root problem with active decentralized adversaries---the higher influence factor induced by sparse communication topologies.
 %However, secure aggregation cannot reduce the	higher influence factor induced by sparse communication topologies (see Section~\ref{sec:influence_factor}) and hence cannot prevent all attacks by active decentralized adversaries.

\parabf{Robust aggregation.}
Robust aggregation methods~\cite{karimireddy2021learning} are neither a good defense against privacy attacks (we show this in Appendix~\ref{app:selfclip}). 
%In general, robust aggregation techniques can only trade privacy for robustness as they either magnify the influence of the local training, leaking information; or protect this information by letting model updates provided by neighbors influence the local training (see the effect of echo attacks on self-centering clipping~\cite{he2022byzantine} in Section~\ref{app:selfclip}).
In general, robust aggregation techniques can only trade privacy for robustness and \textit{viceversa} as they either magnify the influence of external sources of information (\ie model updates provided by neighbors) or internal ones  (\ie the current state of the model).
%In general, robust aggregation techniques can only trade privacy for robustness as they  magnify the influence internal ones  (\ie the current state of the model).
	 
We acknowledge that robust aggregations can hamper attacks such as the state-override attack. However, robust aggregation protocols also apply to the federated settings {(see Appendix~\ref{app:fl_and_robustagg} for a detailed discussion)}. Therefore, this defense simply does not close the security gap between DL and FL.

% See Appendix~\ref{app:selfclip} for more details.



==> torus_scheme.tex <==
\begin{tikzpicture}
	\centering
	%\clip (-1,-1) rectangle (6cm,6cm); 
	\draw[style=help lines,thick] (0,0) grid[step=.5cm] (1,1);
	
	\foreach \x in {0,1,...,2}
	{
		\foreach \y in {0,1,...,2}
		{
			\node[draw,circle,inner sep=2pt,fill] at (.5*\x,.5*\y) {};
		}
	}
\end{tikzpicture}
